High Speed and High Dynamic Range Video with an Event Camera

Event cameras are novel sensors that report brightness changes in the form of a stream of asynchronous "events" instead of intensity frames. They offer significant advantages with respect to conventional cameras: high temporal resolution, high dynamic range, and no motion blur. While the stream of events encodes in principle the complete visual signal, the reconstruction of an intensity image from a stream of events is an ill-posed problem in practice. Existing reconstruction approaches are based on hand-crafted priors and strong assumptions about the imaging process as well as the statistics of natural images. In this work we propose to learn to reconstruct intensity images from event streams directly from data instead of relying on any hand-crafted priors. We propose a novel recurrent network to reconstruct videos from a stream of events, and train it on a large amount of simulated event data. During training we propose to use a perceptual loss to encourage reconstructions to follow natural image statistics. We further extend our approach to synthesize color images from color event streams. Our network surpasses state-of-the-art reconstruction methods by a large margin in terms of image quality (> 20%), while comfortably running in real-time. We show that the network is able to synthesize high framerate videos (> 5,000 frames per second) of high-speed phenomena (e.g. a bullet hitting an object) and is able to provide high dynamic range reconstructions in challenging lighting conditions. We also demonstrate the effectiveness of our reconstructions as an intermediate representation for event data. We show that off-the-shelf computer vision algorithms can be applied to our reconstructions for tasks such as object classification and visual-inertial odometry and that this strategy consistently outperforms algorithms that were specifically designed for event data.

==> chapters/__latexindent_temp.tex <==
\IEEEtitleabstractindextext{%
\begin{abstract}
Event cameras are novel sensors that report brightness changes in the form of asynchronous ``events'' instead of intensity frames.
They have significant advantages over conventional cameras: high temporal resolution, high dynamic range, and no motion blur.
Since the output of event cameras is fundamentally different from conventional cameras, it is commonly accepted that they require the development of specialized algorithms to accommodate the particular nature of events.
In this work, we take a different view and propose to apply existing, mature computer vision techniques to videos reconstructed from event data.
We propose a novel recurrent network to reconstruct videos from a stream of events, and train it on a large amount of simulated event data.
Our experiments show that our approach surpasses state-of-the-art reconstruction methods by a large margin ($>\!20\%$) in terms of image quality, \revised{while running comfortably in real-time ($\ge 200$ Hz on GPU)}.
We further apply off-the-shelf computer vision algorithms to videos
reconstructed from event data on tasks such as object classification and visual-inertial odometry, and show that this strategy consistently outperforms algorithms that were specifically designed for event data.
We believe that our approach opens the door to bringing the outstanding properties of event cameras to an entirely new range of tasks. %
A video of the experiments is available at \url{https://youtu.be/xxxxxxxx}
\end{abstract}

\begin{IEEEkeywords}
    Event-based vision, Dynamic Vision Sensor, Video Reconstruction, High-Speed Imaging
    \end{IEEEkeywords}

}


==> figures/fig_bayer.tex <==
\global\long\def\bayerHeight{3.2cm} %
\begin{figure}[t]
	\centering
	\begin{tabular}{cc}
	\includegraphics[height=\bayerHeight]{images/bayer/RGBG.pdf}
	\hspace{1pt}
    & \includegraphics[height=\bayerHeight]{images/bayer/color_events.png}
	\end{tabular}
	\caption{Left: 2$\times$2 RGBG Bayer pattern in the Color-DAVIS346.
		Right: Events from the Color-DAVIS346 split into each color.
		Positive (ON) events are colored by the corresponding filter color, negative (OFF) events are black.
	}
	\label{fig:bayer}
\end{figure}%


==> figures/fig_network_memory.tex <==
\global\long\def\heightplot{2.55cm} %
\global\long\def\widthplot{3.4cm} %
\begin{figure*}
	\centering
    \begin{tabular}{ccccc}
    \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_LRT_HDR/dynamic_6dof/frame_0000000049.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_LRT_HDR/dynamic_6dof/frame_0000000149.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_LRT_HDR/dynamic_6dof/frame_0000000299.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_LRT_HDR/dynamic_6dof/frame_0000000549.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_LRT_HDR/dynamic_6dof/frame_0000001049.png}\\
    (a) Initial time & (b) After 100 iterations & (c) After 250 iterations & (d) After 500 iterations & (e) After 1000 iterations
    \end{tabular}
\caption{How large is the memory of our network? As in Fig.~\ref{fig:network_memory_comp}, the events are artificially stopped at some time $t$, \ie the network is fed empty event tensors in all the next iterations.
By contrast to Fig.~\ref{fig:network_memory_comp}, we analyze the network behavior on a much larger temporal scale (one to two orders of magnitude more iterations).
After a few hundred empty tensors, the network starts diverging, and produces artefacts.
}
\label{fig:network_memory}
\end{figure*}

==> figures/fig_network_memory_comp.tex <==
\global\long\def\heightplot{2.55cm} %
\global\long\def\widthplot{3.4cm} %
\begin{figure*}
	\centering
    \begin{tabular}{ccccc}

    \rotatebox{90}{RNN}
    \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_short_range/dynamic_6dof/frame_0000000049.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_short_range/dynamic_6dof/frame_0000000054.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_short_range/dynamic_6dof/frame_0000000059.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_short_range/dynamic_6dof/frame_0000000064.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_short_range/dynamic_6dof/frame_0000000069.png}\\

    \rotatebox{90}{Ours}
    \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_short_range_LRT_HDR/dynamic_6dof/frame_0000000049.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_short_range_LRT_HDR/dynamic_6dof/frame_0000000054.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_short_range_LRT_HDR/dynamic_6dof/frame_0000000059.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_short_range_LRT_HDR/dynamic_6dof/frame_0000000064.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/limitations/limited_memory_short_range_LRT_HDR/dynamic_6dof/frame_0000000069.png}\\

    (a) Initial time & (b) After 5 iterations & (c) After 10 iterations & (d) After 15 iterations & (e) After 20 iterations\\



    \end{tabular}
\caption{Comparing the size of our network's memory against the vanilla RNN \cite{Rebecq19cvpr}.
In this experiment, the events are artificially stopped at some time $t$, \ie both networks are fed empty event tensors in all the next iterations.
The correct thing to do would be to simply copy the first image to all the next image predictions.
In fact, this is indeed what both network do in the first iterations.
However, after just a few empty tensors, the vanilla RNN \cite{Rebecq19cvpr} network gradually fades the reconstructions away, while our network can preserve the reconstructions much better, thanks
to the stacked ConvLSTMs used in the encoders, and the longer training sequences.
}
\label{fig:network_memory_comp}
\end{figure*}

==> figures/fig_qualitative_night.tex <==
\setlength{\tabcolsep}{0.15ex} %
\global\long\def\heightplot{1,852cm} %
\global\long\def\widthplot{2.71cm} %
\begin{figure}
	\centering
    \begin{tabular}{ccc}
    \includegraphics[width=\widthplot,height=\heightplot]{images/qualitative/MVSEC/night/1098_VISENSOR.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/qualitative/MVSEC/night/1098_events.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/qualitative/MVSEC/night/1098_reconstructed_LRT_HDR.png}\\
    \footnotesize (a) VI Sensor & \footnotesize (b) Events & \footnotesize (c) Our reconstruction
    \end{tabular}
\caption{A high-dynamic-range reconstruction from an event camera mounted on a car driving at night \cite{Zhu18ral}.
Because of low light, the conventional camera image is severely degraded (a).
In contrast, the events (b) capture the whole dynamic range of the scene, which our method successfully converts into an image (c), recovering details that are lost in the conventional frame. %
}
\label{fig:qualitative_night}
\end{figure}

==> figures/fig_zoom_hdr_reconstructions.tex <==
\global\long\def\heightplot{2.5cm} %
\global\long\def\widthplot{2.5cm} %
\setlength{\tabcolsep}{0.05cm} %
\begin{figure}
	\centering
    \begin{tabular}{ccc}

    \rotatebox{90}{VI sensor}
    \includegraphics[width=\widthplot,height=\heightplot]{images/qualitative/MVSEC/hdr/163_VISENSOR_zoom.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/qualitative/MVSEC/night/1098_VISENSOR_zoom.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/qualitative/MVSEC/night/1098_VISENSOR_zoom2.png}\\[\vspacecols]

    \rotatebox{90}{Ours}
    \includegraphics[width=\widthplot,height=\heightplot]{images/qualitative/MVSEC/hdr/163_reconstructed_LRT_HDR_zoom.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/qualitative/MVSEC/night/1098_reconstructed_LRT_HDR_zoom.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/qualitative/MVSEC/night/1098_reconstructed_LRT_HDR_zoom2.png}\\[\vspacecols]



    (a) Day & (b) Night 1 & (c) Night 2 \\
    \end{tabular}
\caption{Zoom on two reconstructions from Fig.~\ref{fig:hdr_reconstructions}.
The images from the VI sensor (first row) either suffer from over exposure when the camera is facing the sun (a), or under-exposure at night time (b,c).
In contrast, our reconstructions from event data (second row) have a higher dynamic range, and reveal details that were lost in the regular image.
Note that the DAVIS346 used has lower resolution ($346 \times 260$ pixels) than the VI sensor (VGA resolution).
}
\label{fig:zoom_hdr_reconstructions}
\end{figure}


==> figures/fig_zoom_highspeed_reconstructions.tex <==
\global\long\def\heightplot{3.5cm} %
\global\long\def\widthplot{3.5cm} %
\setlength{\tabcolsep}{0.2cm} %

\begin{figure*}
	\centering
    \begin{tabular}{cccc}

    \includegraphics[width=\widthplot,height=\heightplot]{images/qualitative/high_speed/gnome/gnome_zoom_sharp.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/qualitative/high_speed/mug/mug_zoom_sharp.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/qualitative/high_speed/water_balloon/water_balloon_zoom_sharp.png}
    & \includegraphics[width=\widthplot,height=\heightplot]{images/qualitative/high_speed/balloon/balloon_zoom_sharp.png}\\

    (a) Gnome & (b) Mug & (c) Water balloon & (d) Air balloon\\

    \end{tabular}

\caption{Zoom on some stills from our high speed video reconstructions.
In (a) and (b), the trace of the bullet is clearly visible (although the bullet itself was too fast even for the event sensor to catch), 
and cracks in both objects are visible, right before they are being shattered.
In (c) and (d), the membrane of the balloons contracting away from the point where the needle hit is clearly visible.
In (d), the ``ghost'' of the balloon is still visible, which is a failure case of our reconstruction.
}
\label{fig:zoom_high_speed_reconstructions}
\end{figure*}

